A Unifying Generative Model for Graph Learning Algorithms: Label Propagation, Graph Convolutions, and Combinations

Semi-supervised learning on graphs is a widely applicable problem in network science and machine learning. Two standard algorithms -- label propagation and graph neural networks -- both operate by repeatedly passing information along edges, the former by passing labels and the latter by passing node features, modulated by neural networks. These two types of algorithms have largely developed separately, and there is little understanding about the structure of network data that would make one of these approaches work particularly well compared to the other or when the approaches can be meaningfully combined. Here, we develop a Markov random field model for the data generation process of node attributes, based on correlations of attributes on and between vertices, that motivates and unifies these algorithmic approaches. We show that label propagation, a linearized graph convolutional network, and their combination can all be derived as conditional expectations under our model, when conditioning on different attributes. In addition, the data model highlights deficiencies in existing graph neural networks (while producing new algorithmic solutions), serves as a rigorous statistical framework for understanding graph learning issues such as over-smoothing, creates a testbed for evaluating inductive learning performance, and provides a way to sample graphs attributes that resemble empirical data. We also find that a new algorithm derived from our data generation model, which we call a Linear Graph Convolution, performs extremely well in practice on empirical data, and provide theoretical justification for why this is the case.

==> paper/background.tex <==
% !TEX root = ../main.tex

\section{Review of Label Propagation and Graph Convolution Network}
%
\textbf{Label propagation} is a transductive learning method based on the fact that adjacent vertices tend to have similar labels.
%
For regression or binary classification ($-1$ or $+1$), let $\vf^{(0)} \in \mathbb{R}^{n}$ denote the initial beliefs with $f_{u}^{(0)} = y_{u}$ the ground truth label for $u \in L$ and $f_{u}^{(0)} = 0$ otherwise, the final beliefs are computed iteratively,
%
\begin{align}
    \forall u \in V.\quad f_{u}^{(t+1)} \leftarrow (1 - \alpha) \cdot f_{u}^{(0)} + \alpha \cdot d_{u}^{-1/2} \sum_{v \in N(u)} d_{v}^{-1/2} f_{v}^{(t)}
    \label{eq:lp}
\end{align}
%
where $d_{u}$ is the degree of vertex $u$ and $\alpha$ is a mixing parameter.
%
It has been shown that the stationary point of \cref{eq:lp} minimize the following objective function~\cite{Zhou_2004},
%
\begin{align}
    \vy^{*, \rm LPA} = \arg\min_{\vf} \mathcal{Q}(\vf) = \arg\min_{\vf} \left(\mu \cdot \|\vf - \vf^{(0)}\|^{2} + \vf^{\intercal} \mN \vf\right)
    \label{eq:lp_objective}
\end{align}
%
where $\mu = (1-\alpha) / \alpha$ and $\mN$ is the normalized Laplacian matrix.

 Label propagation easily generalizes to classification setting with $c > 2$ classes.

 Let $\bar{\mathbf{p}}_{u} \in \mathbb{R}^{c}$ denote the initial belief vector for the probabilities of vertex $u$ in different classes, the probability of each class is propagated separately in each dimension to get the final beliefs.
 %
 \begin{align}
     \bm{p}_{u}^{(t+1)} \leftarrow (1 - \lambda) \cdot \bar{\mathbf{p}}_{u} + \lambda \cdot d_{u}^{-1/2} \sum_{v \in N(u)} d_{v}^{-1/2} \bm{p}_{v}^{(t)}
     \label{eq:lp}
 \end{align}

\textbf{GCN}, on the other hand, is an inductive learning method that learns a mapping from features in the neighborhood of a vertex to its label.
%
A $K$-layer GCN predicts the vertex labels as follows,
%
\begin{align}
    \vy^{*, \rm GCN} &= f(\tilde{\mS}\ldots \sigma(\tilde{\mS}\mX\Theta^{(1)})\ldots\Theta^{(K)})
    \label{eq:gcn}
\end{align}
%
where $\sigma$ is the activation function, $f$ is the output function, $\Theta^{(k)}$ is the neural network weights at layer-$k$, and $\tilde{\mS} = (\mD + \mathbf{I})^{-1/2} (\mW + \mathbf{I}) (\mD + \mathbf{I})^{-1/2}$ is the normalized adjacency matrix with self-loops.
%
In particular, if both the activation and output functions are linear (\textit{i.e.} $\sigma(x) = x$, $f(\vx) = \vx^{\intercal} \beta_{0}$),
%
\begin{align}
    \vy^{*, \rm SGC} = \tilde{\mS}^{K} \mX \Theta^{(1)} \ldots \Theta^{(K)} \beta_{0} = \tilde{\mS}^{K} \mX \beta
    \label{eq:sgc}
\end{align}
%
which will be referred as simple graph convolution (SGC)~\cite{Wu_2019} in the following discussion.





==> paper/model_classification.tex <==
\section{Modeling Categorical Attributed Graph as a Discrete MRF}
%
Finally, we note the label propagation solution in \cref{eq:lp_conditional} can be written using the normalized adjacency matrix $\mW = \mD^{-1/2} \mW \mD^{-1/2}$,
%
\begin{align}
    \bar{\vy}_{U} = \left(\mathbf{I} - \frac{\omega}{1 + \omega} \mW\right)_{UU}^{-1} \left[\left(\frac{\omega}{1 + \omega} \mW\right)_{UL} \vy_{L}\right] = \left(\mathbf{I} - \frac{\omega}{1 + \omega} \mW\right)_{UU}^{-1} \widetilde{\vy}_{U}
    \label{eq:lp_conditional_alternative}
\end{align}
%
where $\widetilde{\vy}_{U}$ can be viewed as the ``prior labels'' for the unknown vertices.
%
This expression would be useful later when we consider categorical labels and connect belief propagation with label propagation.

%
Here, we consider the scenario where all the vertex features and labels are categorical.
%
In this case, all attribute values are assumed to be jointly sampled from a discrete MRF,
%
\begin{align}
    p(\bm{A}) = \frac{H(\bm{A})}{\sum_{\bm{A}'} H(\bm{A}')} = \frac{\left[\prod_{(u,v) \in E} \prod_{i=1}^{q+1} \phi_{i}(a_{ui}, a_{vi})\right] \left[\prod_{u \in V} \prod_{i<j}^{q+1} \psi_{ij}(a_{ui}, a_{uj})\right]}{Z}
    \label{eq:mrf}
\end{align}
%
where $\phi_{i}$ encodes the homophily of type-$i$ attribute on neighboring vertices, $\psi_{ij}$ encodes the correlation between type-$i$ and type-$j$ attributes on the same vertex, and $Z = \sum_{\bm{A}'} H(\bm{A}')$ is a normalization constant.
%
We require $\phi_{i}(\cdot,\cdot)$ to be symmetric functions.
%
Since the attributes take discrete classes, the pair potentials $\phi_{i}$ and $\psi_{ij}$ each takes a finite number of discrete values, which we group into coupling matrices $\Phi_{i} \in \mathbb{R}^{c_{i} \times c_{i}}$ and $\Psi_{ij} \in \mathbb{R}^{c_{i} \times c_{j}}$ respectively, where $c_{i}$ is number of classes for attribute $i$.
%
Next, we are going to assume the pair potentials are known apriori, and our goal is to estimate the marginal probabilities of the unknown labels conditioned on the predictors.
%
We will first prove the conditional distribution of $\bm{y}_{U}$ is another discrete MRF, then we show the belief propagation algorithm that computes the marginal probabilities $\{\bm{p}_{u}\}_{u \in U}$ are well-approximated by LPA and GCN under suitable assumptions.

\subsection{LPA and GCN Approximate Linearized Belief Propagation on a Discrete MRF}
%
Belief propagation (BP) is a widely used algorithm for computing the marginal probabilities on MRF, which iteratively propagate initial beliefs of random variables throughout the network.
%
However, the original BP algorithm is only guaranteed to converge on tree-structured networks.
%
To this end, Gatterbauer \etal proposed linearized BP (LinBP)~\cite{Gatterbauer_2014}, which provably converges on all networks and empirically gives almost identical prediction as the original BP algorithm.
%
The key idea of LinBP is to expand the MRF potentials and marginal probabilities around some base values and converts the nonlinear BP updates into linear equations.
%
Next, we adapt the LinBP to a special case where the interaction among attributes on neighboring vertices is assumed to be homophily.
%
Our derivation (see \cref{sec:appendix_linbp}) largely follows the original paper and our main result is summarized as follows:
%
\begin{theorem}
Consider a discrete MRF consists of $n$ categorical variables with network topology $G$.
%
The variables are of the same type with $c$ possible classes.
%
The probability distribution is given by,
%
\begin{align}
    p(\bm{y}) = \frac{\left[\prod_{(u,v) \in E} \phi(y_{u}, y_{v})\right] \left[\prod_{u \in V} \varphi_{u}(y_{u})\right]}{Z}
    \label{eq:linbp_mrf}
\end{align}
%
where $\varphi_{u}(\cdot)$ is the self-potential for variable $y_{u}$.
%
Note the joint probability in \cref{eq:linbp_mrf} is invariant with respect to a constant scaling of the potentials.
%
Without loss of generality, let us denote:
%
\begin{itemize}[leftmargin=0.2in]
    \item $\mathbf{W} \in \mathbb{R}^{n \times n}$ the adjacency matrix for graph $G$
    \item $\mathbf{J}_{c} \in \mathbb{R}^{c \times c}$ the constant-$1$ matrix, \enskip $\mathbf{1}_{c} \in \mathbb{R}^{c}$ the constant-$1$ vector
    \item $\Phi \in \mathbb{R}^{c \times c}$ the symmetric coupling matrix (scaled to have each row/column with mean value $1$)
    \item $\varphi_{u} \in \mathbb{R}^{c}$ the self-potential vector for $y_{u}$ (scaled to sum to $1$), interpreted as prior probabilities
    \item $\bm{p}_{u} \in \mathbb{R}^{c}$ the marginal probability vector for $y_{u}$
\end{itemize}
%
Next, define base values for potentials/probabilities, and residuals as deviation from base values,
%
\begin{itemize}[leftmargin=0.2in]
    \item $\Phi_{0} = \eta \cdot \mathbf{J}_{c}$ the base coupling matrix, \enskip $\hat{\Phi} = \Phi - \Phi_{0}$ the residual coupling matrix
    \item $\varphi_{0} = \frac{1}{c} \cdot \mathbf{1}_{c}$ the base prior vector, \enskip $\hat{\varphi}_{u} = \varphi_{u} - \varphi_{0}$ the residual prior vector for $y_{u}$
    \item $\bm{p}_{0} = \frac{1}{c} \cdot \mathbf{1}_{c}$ the base probability vector, \enskip $\hat{\bm{p}}_{u} = \bm{p}_{u} - \bm{p}_{0}$ the residual probability vector for $y_{u}$
\end{itemize}
%
We assume the interaction between attributes on neighboring vertices is homophily.
%
In particular, let $\eta = \left(1 - \frac{\epsilon}{c}\right)$ and $\hat{\Phi} = \epsilon \mathbf{I}_{c}$ for a small positive constant $\epsilon$, then the LinBP algorithm computes the residual probability vectors iteratively until convergence,
%
\begin{align}
    \hat{\bm{p}}_{u}^{(t+1)} \leftarrow \hat{\varphi}_{u} + \frac{\epsilon}{c} \sum_{v \in \mathcal{N}(u)} \hat{\bm{p}}_{v}^{(t)}
    \label{eq:linbp}
\end{align}
%
Let $\hat{\varphi} = [\hat{\varphi}_{1}, \ldots, \hat{\varphi}_{n}]$ and $\hat{\bm{p}} = [\hat{\bm{p}}_{1}, \ldots, \hat{\bm{p}}_{n}]$, the stationary point solution for \cref{eq:linbp} is given by,
%
\begin{align}
    \hat{\bm{p}} = \left(\mathbf{I} - \frac{\epsilon}{c} \cdot \mathbf{W} \otimes \mathbf{I}_{c}\right)^{-1} \hat{\varphi}
    \label{eq:linbp_solution}
\end{align}
%
\end{theorem}
%
% The residual coupling matrix $\hat{\Phi}$ in \cref{eq:linbp} makes explicit the relative attraction and repulsion across the graph: $\hat{\Phi}(k,l) > 0$ indicates it is favorable to have one variable in class $k$ neighboring another variable in class $l$, and $\hat{\Phi}(k,l) < 0$ indicates the opposite.
%
% For categorical variables with homophily interactions, $\hat{\Phi}$ is positive along its diagonal and negative on the off-diagonal.
%
% On the other hand, 
%
It is worth noting that the residual prior $\hat{\varphi}_{u}$ gives the initial \emph{local} preference of $y_{u}$ for each class.
%
Next, we are going to model different types of data with \cref{eq:mrf}.
%
We show the LinBP algorithm that compute the marginal probabilities of unknown labels reduces to LPA and LinGCN starting with different residual priors.

\xhdr{Case 1: label propagation for label-only graph data}
%
In this case, \cref{eq:mrf} can be simplified as:
%
\begin{align}
    p(\bm{y}) = \frac{\prod_{(u,v) \in E} \phi(y_{u}, y_{v})}{Z}
    \label{eq:mrf_labels}
\end{align}
%
where we have dropped the attribute type index $i$.
%
The joint distribution of $\bm{y}_{U}$ given $\bm{y}_{L} = \mathbf{y}_{L}$ is,
%
\begin{align}
    p(\bm{y}_{U}|\bm{y}_{L}=\mathbf{y}_{L})
    &= \frac{\left[\prod_{u \in U} \prod_{v \in \mathcal{N}(u) \cap U} \phi(y_{u}, y_{v})\right] \left[\prod_{u \in U} \prod_{v \in \mathcal{N}(u) \cap L} \phi(y_{u}, \mathrm{y}_{v})\right]}{Z} \nonumber \\
    &= \frac{\left[\prod_{u \in U} \prod_{v \in \mathcal{N}(u) \cap U} \phi(y_{u}, y_{v})\right] \prod_{u \in U} \varphi_{u}^{0}(y_{u})}{Z}
    \label{eq:mrf_unknown_labels}
\end{align}
%
where $\varphi_{u}^{0}(k) = \prod_{v \in \mathcal{N}(u) \cap L} \phi(k, \mathrm{y}_{v})$ can be further normalized as $\varphi_{u}(k) = \varphi_{u}^{0}(k) / \sum_{l=1}^{c} \varphi_{u}^{0}(l)$.
%
We note that the conditional distribution of $\bm{y}_{U}$ is still a MRF, and conditioning on $\bm{y}_{L} = \mathbf{y}_{L}$ effectively introduces prior beliefs to $\{y_{u}\}_{u \in U}$.
%
Moreover, the MRF adjacency matrix for \cref{eq:mrf_unknown_labels} is $\mathbf{W}_{UU}$, the principle submatrix for the MRF adjacency matrix in \cref{eq:mrf_labels}.
%
Denote $\hat{\varphi}_{U} = [\hat{\varphi}_{u}]_{u \in U}$ and $\hat{\bm{p}}_{U} = [\hat{\bm{p}}_{u}]_{u \in U}$, we can use LinBP algorithm to compute the marginal probabilities,
%
% First, the update equation of label propagation \cref{eq:lp} and that of LinBP \cref{eq:linbp} both iteratively compute the next step's belief with the prior belief and the current beliefs of the neighbors.
%
% The two algorithms only differ in how they combine prior and current beliefs --- label propagation computes new belief as the weighted average of the prior and current beliefs, while LinBP updates the prior with influence from the current belief.
%
% Moreover, assume the interactions between neighboring labels are homophily and $\Phi = \left(1 - \frac{\epsilon}{c}\right) \cdot \mathbf{J}_{c} + \epsilon \cdot \mathbf{I}_{c}$ is the coupling matrix, LinBP solution \cref{eq:linbp_solution} becomes,
%
\begin{align}
    \hat{\bm{p}}_{U} = \left(\mathbf{I} - \frac{\epsilon}{c} \cdot \mathbf{W}_{UU} \otimes \mathbf{I}_{c}\right)^{-1} \hat{\varphi}_{U}
    \label{eq:linbp_solution_homophily}
\end{align}
%
Now let us compare \cref{eq:linbp_solution_homophily} with the solution of label propagation \cref{eq:lp_conditional_alternative}.
%
Note $(\mathbf{I} - \frac{\epsilon}{c} \cdot \mathbf{W}_{UU} \otimes \mathbf{I}_{c})$ is psychologically block diagonal, and so is its inverse.
%
Therefore, \cref{eq:linbp_solution_homophily} can be viewed as applying $(\mathbf{I} - \frac{\epsilon}{c} \cdot \mathbf{W})_{UU}^{-1}$ to propagate the residual probability of each class independently.
%
It only differs from \cref{eq:lp_conditional_alternative} in that it uses the unnormalized adjacency matrix $\mathbf{W}$ instead of the normalized one $\mathcal{W}$.
%
Finally, we assume $\epsilon$ is a small constant and linearize the prior belief $\varphi_{u}^{0}$ using $(1+\epsilon)^{d} \approx 1+d\epsilon$,
%
\begin{align}
    \varphi_{u}^{0}(k) = \prod_{v \in \mathcal{N}(u) \cap L} \left(1-c^{-1}\epsilon\right)^{1-\delta_{k \mathrm{y}_{v}}} \left(1-c^{-1}\epsilon+\epsilon\right)^{\delta_{k \mathrm{y}_{v}}} &\approx \left[1 + \epsilon \left(d_{u}^{L,k} - c^{-1} d_{u}^{L}\right)\right] \nonumber \\
    &\propto \left[1 + \epsilon \left(d_{u}^{L,k} - c^{-1} d_{u}^{L}\right)\right] c^{-1}
    \label{eq:linbp_linearized_prior}
\end{align}
%
where $\delta_{k \mathrm{y}_{v}}$ is the Kronecker delta function, $d_{u}^{L} = |v \in \mathcal{N}(u) \cap L|$ is the number of neighbors of $u$ in $L$, and $d_{u}^{L, k} = \sum_{v \in \mathcal{N}(u) \cap L} \delta_{k \mathrm{y}_{v}}$ is the number of neighbors of $u$ in $L$ with the label $k$.
%
The right-hand-side of \cref{eq:linbp_linearized_prior} prior probability normalizes to $1$, therefore the residual prior,
%
\begin{align}
    \hat{\varphi}_{u}(k) = \varphi_{u}(k) - \varphi_{0}(k) = \frac{\epsilon}{c} \left(d_{u}^{L, k} - c^{-1} d_{u}^{L}\right), \quad \textrm{or equivalently} \enskip \hat{\varphi}_{u} = \frac{\epsilon}{c} \sum_{v \in \mathcal{N}(u) \cap L} \hat{\bm{p}}_{v}
    \label{eq:linbp_linearized_residual_prior}
\end{align}
%
The residual probability $\hat{\bm{p}}_{v} = \bm{p}_{v} - \bm{p}_{0}$, and $\bm{p}_{v}$ is the one-hot encoding of the observed label $y_{v}$.
%
The residual priors $\hat{\varphi}_{u}$ in \cref{eq:linbp_linearized_residual_prior} corresponds to $\widetilde{\mathbf{y}}_{U}$ in \cref{eq:lp_conditional_alternative}, as both are weighted sum over neighbors.

\xhdr{Case 2: GCN for attributed graph data}
%
First, rewrite \cref{eq:mrf} with features $\bm{X}$ and labels $\bm{y}$,
%
\begin{align}
    p(\bm{X}, \bm{y}) = \frac{\left[\prod_{(u,v) \in E} \phi_{q+1}(y_{u}, y_{v})\right] \left[\prod_{u \in V} \prod_{i=1}^{d} \psi_{i,q+1}(x_{ui}, y_{u})\right] H(\bm{X})}{Z}
\end{align}
%
where $H(\bm{X})$ is the part of potential that only involves the features $\bm{X}$.
%
Then, we can compute the joint distribution of the labels $\bm{y}$ given the feature values $\bm{X} = \mathbf{X}$.
%
\begin{align}
    p(\bm{y}|\bm{X}=\mathbf{X}) &= \frac{\left[\prod_{(u,v) \in E} \phi_{q+1}(y_{u}, y_{v})\right] \left[\prod_{u \in V} \prod_{i=1}^{q} \psi_{i,q+1}(\mathrm{x}_{ui}, y_{u})\right]}{Z / H(\mathbf{X})} \nonumber \\
    &= \frac{\left[\prod_{(u,v) \in E} \phi_{q+1}(y_{u}, y_{v})\right] \prod_{u \in V} \varphi_{u}^{0}(y_{u})}{Z'}
\end{align}
%
$\varphi_{u}^{0}(k) = \prod_{i=1}^{d} \psi_{i,q+1}(\mathrm{x}_{ui}, k)$ is the unnormalized prior belief for $y_{u}$.
%
Assume that each coupling matrix $\Psi_{i,q+1}$ is scaled so that every column has mean value $1$, and each element can be written as $\psi_{i,q+1}(\cdot,\cdot) = 1 + \hat{\psi}_{i,q+1}(\cdot,\cdot)$ with a small residual $\hat{\psi}_{i,q+1}$, then we can linearize $\varphi_{u}^{0}(k)$ as follows:
%
\begin{align}
    \varphi_{u}^{0}(k) = \prod_{i=1}^{q} \left(1 + \hat{\psi}_{i,q+1}(\mathrm{x}_{ui}, k)\right) &\approx 1 + \sum_{i=1}^{q} \hat{\psi}_{i,q+1}(\mathrm{x}_{ui}, k) \nonumber \\
    &\propto \left(1 + \sum_{i=1}^{q} \hat{\psi}_{i,q+1}(\mathrm{x}_{ui}, k)\right) c^{-1} = \varphi_{u}(k)
\end{align}
%
The residual prior can be computed by,
%
\begin{align}
    \hat{\varphi}_{u}(k) = \varphi_{u}(k) - \varphi_{0}(k) = c^{-1} \sum_{i=1}^{q} \hat{\psi}_{i,q+1}(\mathrm{x}_{ui}, k)
    \label{eq:linbp_linearized_residual_prior_attributed_graph}
\end{align}
%
Then, we can use LinBP to compute the marginal probabilities of the labels,
%
\begin{align}
    \hat{\bm{p}} = \left(\mathbf{I} - \frac{\epsilon}{c} \cdot \mathbf{W} \otimes \mathbf{I}_{c}\right)^{-1} \hat{\varphi}
    \label{eq:linbp_solution_attributed_graph}
\end{align}
%
which first computes the residual priors from the features and then smooth the probability of each class independently along the graph topology.
%
However, \cref{eq:linbp_linearized_residual_prior_attributed_graph,eq:linbp_solution_attributed_graph} is not directly applicable to real-world classification tasks, since the coupling matrices $\Psi_{i,q+1}$ are unknown.
%
Nonetheless, it motivates a 3-step inference algorithm 1) compute the hidden representation $\mathbf{z}_{u} = f(\mathbf{x}_{u})$ for every vertex 2) compute smoothed hidden representations $\{\bar{\mathbf{z}}_{u}\}_{u \in V}$ by smoothing $\{\mathbf{z}_{u}\}_{u \in V}$ along the graph topology 3) compute the predictive probabilities as $\mathbf{p}_{u} = g(\bar{\mathbf{z}}_{u})$, where $f, g$ are parametrized with neural networks and trained end-to-end on observed labels.
%
Furthermore, if $f$ is chosen as a linear function (such as \cref{eq:linbp_linearized_residual_prior_attributed_graph}) and $g$ as a simple softmax output layer, then by swapping the transformation step 1 and smoothing step 2 we get LinGCN for classification.

\xhdr{Case 3: GCN with LP probability as additional input}
%
Next, we consider the joint distribution of the unknown labels, conditioned on both the features and the known labels.
%
\begin{align}
    p(\bm{y}_{U}|\bm{y}_{L}=\mathbf{y}_{L}, \bm{X}=\mathbf{X})
    &= \frac{\left[\prod_{u \in U} \prod_{v \in \mathcal{N}(u) \cap U} \phi(y_{u}, y_{v})\right] \prod_{u \in U} \varphi_{u}^{0}(y_{u})}{Z}
    \label{eq:mrf_unknown_labels_wf}
\end{align}
%
where the unnormalized prior belief is given by,
%
\begin{align}
    \varphi_{u}^{0}(k) = \prod_{i=1}^{q} \psi_{i,q+1}(\mathrm{x}_{ui}, k) \prod_{v \in \mathcal{N}(u) \cap L} \phi(k, \mathrm{y}_{v}) 
    \label{eq:unnormalized_prior_belief_wf}
\end{align}
%
we can linearize \cref{eq:unnormalized_prior_belief_wf} similarly as before,
%
\begin{align}
    \varphi_{u}^{0}(k) &\approx \left(1 + \sum_{i=1}^{q} \hat{\psi}_{i,q+1}(\mathrm{x}_{ui}, k)\right) \left(1 + \sum_{v \in \mathcal{N}(u) \cap L} \hat{p}_{v}(k)\ \epsilon \right) \nonumber \\
    &\propto \left(1 + \sum_{i=1}^{q} \hat{\psi}_{i,q+1}(\mathrm{x}_{ui}, k)\right) \left(1 + \sum_{v \in \mathcal{N}(u) \cap L} \hat{p}_{v}(k)\ \epsilon \right) c^{-1}
    \label{eq:prior_belief_wf}
\end{align}
%
We note the final expression in \cref{eq:prior_belief_wf} is normalized, therefore the residual prior is given by
%
\begin{align}
    \hat{\varphi}_{u}(k) = \varphi_{u}(k) - \varphi_{0}(k) &= c^{-1} \sum_{i=1}^{q} \hat{\psi}_{i,q+1}(\mathrm{x}_{ui}, k) + c^{-1} \sum_{v \in \mathcal{N}(u) \cap L} \hat{p}_{v}(k)\ \nonumber \\
    &= \hat{\varphi}_{u}^{\rm features}(k) + \hat{\varphi}_{u}^{\rm labels}(k)
    \label{eq:residual_prior_belief_wf}
\end{align}
%
where the residual prior is split into two parts: $\hat{\varphi}_{u}^{\rm features}$ captures the influences from the features on vertex $u$, while $\hat{\varphi}_{u}^{\rm labels}$ captures the influences from the labels on vertices neighboring to $u$.
%
We can use LinBP to compute the marginal probability of the unknown labels,
%
\begin{align}
    \hat{\bm{p}} = \left(\mathbf{I} - \frac{\epsilon}{c} \cdot \mathbf{W}_{UU} \otimes \mathbf{I}_{c}\right)^{-1} (\hat{\varphi}^{\rm features} + \hat{\varphi}^{\rm labels})
    \label{eq:linbp_solution_attributed_graph_wr}
\end{align}
%
Comparing with \cref{eq:linbp_solution_attributed_graph}, this suggests adding predictive LP probabilities as an additional source of information to the LinGCN algorithm.
%
Specifically, in step 3) of LinGCN, the LPA predictive probabilities on each vertex is used as additional input $\mathbf{p}_{u} = g(\bar{\mathbf{z}}_{u}, \mathbf{p}_{u}^{\rm LPA})$.
%
This additional input also require modification to the LinGCN training process: at each step, we sample a mini-batch $M \subseteq L$; $M$ must be masked as unknown when we run the label propagation algorithm to compute $\{\mathbf{p}_{u}^{\rm LPA}\}_{u \in M}$ to prevent label leakage.
%
This also means we need to rerun label propagation for every LinGCN training step.
%
The performance of this algorithm is tested in \cref{sec:experiments}.

\section{Semi-supervised Classification Performances on Categorical Attributed Graphs}
%
\xhdr{Citation networks}
%
We consider 3 benchmark datasets --- Cora, CiteSeer, and PubMed --- where vertices are articles and edges are citations.
%
The vertex features is given by a vector indicating the absence/presence of a dictionary of words.
%
The goal is to classify each article into different subjects.

\xhdr{WikiCS networks}
%
The dataset consists of nodes corresponding to Computer Science articles, and edges based on hyperlinks.
%
The features each article is calculated as the average of the pretrained GloVe word embeddings in each corresponding article.
%
The goal is to classify each article into 1 of the 10 subfields.
%
\begin{table*}[h]
    \caption{Semi-supervised classification performance on graphs with categorical attributes.}
    \centering
    \resizebox{0.9\linewidth}{!}{
    \begin{tabular}{rlccccccc}
    \toprule
    Dataset       & LR           & LP           & LinGCN       & SGC          & GCN          & LinGCN+      & SGC+         & GCN+         \\
    \midrule
    Cora          & $\nrm{62.5}$ & $\nrm{75.8}$ & $\nrm{83.8}$ & $\nrm{82.6}$ & $\nrm{82.5}$ & $\nrm{83.6}$ & $\nrm{82.6}$ & $\nrm{82.5}$ \\
    CiteSeer      & $\nrm{63.5}$ & $\nrm{55.2}$ & $\nrm{69.6}$ & $\nrm{69.9}$ & $\nrm{69.8}$ & $\nrm{68.8}$ & $\nrm{69.3}$ & $\nrm{69.0}$ \\
    PubMed        & $\nrm{81.8}$ & $\nrm{80.5}$ & $\nrm{85.3}$ & $\nrm{84.9}$ & $\nrm{85.1}$ & $\nrm{85.2}$ & $\nrm{84.8}$ & $\nrm{85.1}$ \\
    WikiCS        & $\nrm{73.6}$ & $\nrm{72.6}$ & $\nrm{75.9}$ & $\nrm{77.2}$ & $\nrm{75.2}$ & $\nrm{76.7}$ & $\nrm{77.8}$ & $\nrm{76.0}$ \\
    \midrule                                                                                                                              
    Cora(10)      & $\nrm{53.6}$ & $\nrm{75.8}$ & $\nrm{74.5}$ & $\nrm{70.5}$ & $\nrm{70.7}$ & $\nrm{77.4}$ & $\nrm{75.1}$ & $\nrm{74.8}$ \\
    CiteSeer(10)  & $\nrm{64.2}$ & $\nrm{55.2}$ & $\nrm{70.0}$ & $\nrm{69.9}$ & $\nrm{70.3}$ & $\nrm{70.2}$ & $\nrm{70.6}$ & $\nrm{70.9}$ \\
    PubMed(10)    & $\nrm{79.4}$ & $\nrm{80.5}$ & $\nrm{82.1}$ & $\nrm{81.5}$ & $\nrm{82.5}$ & $\nrm{82.7}$ & $\nrm{82.5}$ & $\nrm{83.1}$ \\
    WikiCS(10)    & $\nrm{64.1}$ & $\nrm{72.6}$ & $\nrm{74.4}$ & $\nrm{74.8}$ & $\nrm{74.4}$ & $\nrm{75.4}$ & $\nrm{75.5}$ & $\nrm{75.2}$ \\
    \bottomrule
    \end{tabular}
    }
    \label{tab:classification_accuracies}
\end{table*}
%
Next, we shift our the semi-supervised classification setting and test the performance of logistic regression (LR), LPA, LinGCN, SGC, and GCN on several benchmark datasets.
%
Additionally, we test the algorithm given by \cref{eq:linbp_solution_attributed_graph_wr}, which motivate adding the LPA predictive probabilities to the final layer of LinGCN, SGC, and GCN, right before the softmax output function is applied.
%
These augmented algorithms are denoted as LinGCN+, SGC+, and GCN+ respectively.
%
Furthermore, for each attributed graph, we consider a version of the dataset with reduced feature information by compressing the word feature vectors into a low-dimensional real-valued vector space using the principle component analysis.
%
The prediction accuracies of different semi-supervised learning algorithms is reported in \cref{tab:classification_accuracies}.
%
On the original benchmark datasets, we find LinGCN, SGC, and GCN already give high prediction accuracy and incorporating the LPA predictive probabilities gives little additional gains.
%
However, on the datasets with compressed features, the performance of LinGCN, SGC, GCN are on par with LPA, and combing feature information with LPA predictive probabilities improves the predictive performances (sometime by a large margin).

\section{Derivation for Linear Belief Propagation \label{sec:appendix_linbp}}
%
The original belief propagation updates are given as follows:
%
\begin{align*}
    \bm{p}_{u}(k) &\leftarrow \frac{1}{Z_{u}} \varphi_{u}(k) \prod_{v \in \mathcal{N}(u)} \bm{m}_{vu}(k) \\
    \bm{m}_{uv}(k) &\leftarrow \frac{1}{Z_{uv}} \sum_{l} \Phi_{lk} \varphi_{u}(l) \prod_{w \in \mathcal{N}(u) \backslash v} \bm{m}_{wu}(l)
\end{align*}
%
Now, let:
%
\begin{align*}
    \hat{\bm{p}}_{u}(k)  &= \bm{p}_{u}(k)  - \frac{1}{c} \\
    \hat{\bm{m}}_{uv}(k) &= \bm{m}_{uv}(k) - 1           \\
    \hat{\varphi}_{u}(k) &= \varphi_{u}(k) - \frac{1}{c}
\end{align*}
%
We can linearize the first equation as follows:
%
\begin{align*}
    \frac{1}{c} + \hat{\bm{p}}_{u}(k) &\leftarrow \frac{1}{Z_{u}} \cdot \left(\frac{1}{c} + \hat{\varphi}_{u}(k)\right) \cdot \prod_{v \in \mathcal{N}(u)} (1 + \hat{\bm{m}}_{vu}(k)) \\
    \log(1 + c\hat{\bm{p}}_{u}(k)) &\leftarrow -\log Z_{u} + \log \left(1 + c\hat{\varphi}_{u}(k)\right) + \sum_{v \in \mathcal{N}(u)} \log(1 + \hat{\bm{m}}_{vu}(k)) \\
    c\hat{\bm{p}}_{u}(k) &\leftarrow -\log Z_{u} + c\hat{\varphi}_{u}(k) + \sum_{v \in \mathcal{N}(u)} \hat{\bm{m}}_{vu}(k)
\end{align*}
%
Summation both side over $k$, we have:
%
\begin{align*}
    0 \leftarrow -\log Z_{u} + 0 + 0
\end{align*}
%
Therefore, the update equation becomes:
%
\begin{align*}
    \hat{\bm{p}}_{u}(k) \leftarrow \hat{\varphi}_{u}(k) + \frac{1}{c} \cdot \sum_{v \in \mathcal{N}(u)} \hat{\bm{m}}_{vu}(k)
\end{align*}
%
Now, let us look at the second equation,
%
\begin{align*}
    \bm{m}_{uv}(k) &\leftarrow \frac{1}{Z_{uv}} \sum_{l} \Phi_{lk} \varphi_{u}(l) \prod_{w \in \mathcal{N}(u) \backslash v} \bm{m}_{wu}(l) \\
              &\leftarrow \frac{Z_{u}}{Z_{uv}} \sum_{l} \Phi_{lk} \frac{\frac{1}{Z_{u}} \varphi_{u}(l) \prod_{w \in \mathcal{N}(u)} \bm{m}_{wu}(l)}{\bm{m}_{vu}(l)} \\
              &\leftarrow \frac{Z_{u}}{Z_{uv}} \sum_{l} \Phi_{lk} \frac{\bm{p}_{u}(l)}{\bm{m}_{vu}(l)}
\end{align*}
%
Remember $\log Z_{u} = 0$, which means $Z_{u} = 1$.
%
Furthermore, let $\Phi = (1 - \frac{\epsilon}{c}) \mathbf{J} + \epsilon \mathbf{I} = \Phi_{0} + \hat{\Phi}$:
%
\begin{align*}
    1 + \hat{\bm{m}}_{uv}(k) &\leftarrow \frac{1}{Z_{uv}} \sum_{l} \Phi_{lk} \frac{\frac{1}{c} + \hat{\bm{p}}_{u}(l)}{1 + \hat{\bm{m}}_{vu}(l)} \\
                        &\leftarrow \frac{1}{Z_{uv}} \sum_{l} \Phi_{lk} \left(\frac{1}{c} + \hat{\bm{p}}_{u}(l) - \frac{1}{c} \hat{\bm{m}}_{vu}(l)\right) \\
                        &\leftarrow \frac{1}{Z_{uv}} \left(1 + \sum_{l} \Phi_{lk} \hat{\bm{p}}_{u}(l) - \frac{1}{c} \sum_{l} \Phi_{lk} \hat{\bm{m}}_{vu}(l)\right) \\
                        &\leftarrow \frac{1}{Z_{uv}} \left(1 + (\hat{\Phi}\hat{\bm{p}}_{u})(k) - \frac{1}{c} (\hat{\Phi}\hat{\bm{m}}_{vu})(k)\right)
\end{align*}
%
Summation both side over $k$, we have:
%
\begin{align*}
    c + \sum_{k} \hat{\bm{m}}_{uv}(k) &\leftarrow \frac{1}{Z_{uv}} \left(c + \sum_{k} (\hat{\Phi}\hat{\bm{p}}_{u})(k) + \frac{1}{c} \sum_{k} (\hat{\Phi}\hat{\bm{m}}_{vu})(k)\right) \\
                                 &\leftarrow \frac{1}{Z_{ut}} \left(c + \mathbf{1}_{c}^{\intercal}\hat{\Phi}\hat{\bm{p}}_{u} + \mathbf{1}_{c}^{\intercal}\hat{\Phi}\hat{\bm{m}}_{vu}\right) \\
                               c &\leftarrow \frac{1}{Z_{uv}} c
\end{align*}
%
which indicate the normalization factor $Z_{uv} = 1$.
%
Therefore we have:
%
\begin{align*}
    \hat{\bm{m}}_{uv}(k) &\leftarrow (\hat{\Phi}\hat{\bm{p}}_{u})(k) - \frac{1}{c} (\hat{\Phi}\hat{\bm{m}}_{vu})(k) \\
    \hat{\bm{m}}_{uv} &\leftarrow \hat{\Phi}\hat{\bm{p}}_{u} - \frac{1}{c} \hat{\Phi}\hat{\bm{m}}_{vu} \\
    \hat{\bm{m}}_{uv} &\leftarrow \hat{\Phi}\hat{\bm{p}}_{u} - \frac{1}{c} \hat{\Phi}(\hat{\Phi}\hat{\bm{p}}_{v} - \frac{1}{c} \hat{\Phi}\hat{\bm{m}}_{uv}) \\
    \left(\mathbf{I}_{c} - \frac{1}{c^{2}}\hat{\Phi}^{2}\right) \hat{\bm{m}}_{uv} &\leftarrow \hat{\Phi}\hat{\bm{p}}_{u} - \frac{1}{c} \hat{\Phi}^{2}\hat{\bm{p}}_{v}
\end{align*}
%
At convergence, we have:
%
\begin{align*}
    \hat{\bm{m}}_{uv} = \left(\mathbf{I}_{c} - \frac{1}{c^{2}}\hat{\Phi}^{2}\right)^{-1} \left(\hat{\Phi}\hat{\bm{p}}_{u} - \frac{1}{c} \hat{\Phi}^{2} \hat{\bm{p}}_{v}\right)
\end{align*}
%
Finally, the residual beliefs can be computed by:
%
\begin{align*}
    \hat{\bm{p}}_{u} \leftarrow \hat{\varphi}_{u} + \frac{1}{c} \cdot \sum_{v \in \mathcal{N}(u)} \left(\mathbf{I}_{c} - \frac{1}{c^{2}}\hat{\Phi}^{2}\right)^{-1} \left(\hat{\Phi}\hat{\bm{p}}_{v} - \frac{1}{c} \hat{\Phi}^{2} \hat{\bm{p}}_{u}\right)
\end{align*}
%
Recall $\epsilon$ is small, dropping the second order terms gives:
%
\begin{align*}
    \hat{\bm{p}}_{u} \leftarrow \hat{\varphi}_{u} + \frac{1}{c} \cdot \sum_{v \in \mathcal{N}(u)} \hat{\Phi} \hat{\bm{p}}_{v}
\end{align*}

==> paper/related_work.tex <==
\section{Related Works}
%
\xhdr{Graph-based semi-supervised learning methods}
%
Label propagation methods are originally introduced as semi-supervised learning methods for the \iid data, where a fully connected weighted graph is built from pairwise feature similarities amongst all data points ~\cite{Zhu_2003,Zhou_2004} and the observed labels are diffused along the edges.
%
Later on, when label propagation is adapted for labeled graph data, the relational graph (which oftentimes encode homophily) is used as the topology for label diffusion.
%
However, there has been limited success in directly extending label propagation to account for additional vertex features in attributed graph, as it remains unclear how to combine the feature similarities and relational graph.

\xhdr{Modeling label with conditional random fields}
%
Early semi-supervised learning literatures have considered modeling the labels in a \iid dataset as jointly sampled from a conditional random field where each pair potential is a function of the feature similarities~\cite{Zhu_2002,Zhu_2003,Li_2004}.
%
In particular, for real-valued labels, it has been shown that label propagation gives the mean estimates for the unknown labels in a Gaussian conditional random field~\cite{Zhu_2003}.
%
In contrast to those works, our Markov random field models are designed for attributed graph data: vertex features are explicitly modeled as random variables and the interacting pair potentials are given by the relational graph.


\xhdr{Graph convolutional networks}
%
Graph convolutional networks~\cite{Kipf_2016,Hamilton_2017} are designed to account for the ever growing additional features in attributed graph datasets.
%
GCNs have shown to be able to combine structural and feature information in attributed graph and achieve the state-of-the-art performances on benchmark datasets, however, the factors that contributed to their success are far from understood.
%
Moreover, although the popularity of GCNs has been greatly boosted by the attentions on deep learning methods in general, a lot of recent works suggest that the nonlinearity in GCNs does not contribute much to their performance~\cite{Wu_2019,Li_2019,Liu_2020}.
%
For example, it has been shown that simple graph convolution~\cite{Wu_2019} gives similar performance with the original GCN on some standard benchmark citation networks, indicating the feature smoothing step plays a far more important role than nonlinear transformations.
%
On the other hand, it also has been noted that feature smoothing does not always help and over-smoothing hurts prediction accuracies~\cite{Li_2018,oono2020graph}.
%
To those ends, our proposed Gaussian MRF model provides a theoretically sound rational for feature smoothing, an adjustable parameter to control the smoothing level, as well as a principled way to understand the optimal smoothing level as the balance between homophily strength and noise level.

\begin{itemize}[leftmargin=0.2in]
    \item Collective Inference (not using feature smoothing) [http://eliassi.org/papers/ai-mag-tr08.pdf]
    \item Stats/Sociology (network regression) [Prediction Models For Network-Linked Data]
\end{itemize}

\begin{itemize}[leftmargin=0.2in]
    \item Learning Synthetic Parameters; learned $\gamma$ and empirical $\gamma$
    \item Inductive Graph Neural Network Model
\end{itemize}

